A Minimal Intervention Definition of Reverse Engineering a Neural Circuit

In neuroscience, researchers have developed informal notions of what it means to reverse engineer a system, e.g., being able to model or simulate a system in some sense. A recent influential paper of Jonas and Kording, that examines a microprocessor using techniques from neuroscience, suggests that common techniques to understand neural systems are inadequate. Part of the difficulty, as a previous work of Lazebnik noted, lies in lack of formal language. We provide a theoretical framework for defining reverse engineering of computational systems, motivated by the neuroscience context. Of specific interest are recent works where, increasingly, interventions are being made to alter the function of the neural circuitry to both understand the system and treat disorders. Starting from Lazebnik's viewpoint that understanding a system means you can ``fix it'', and motivated by use-cases in neuroscience, we propose the following requirement on reverse engineering: once an agent claims to have reverse-engineered a neural circuit, they subsequently need to be able to: (a) provide a minimal set of interventions to change the input/output (I/O) behavior of the circuit to a desired behavior; (b) arrive at this minimal set of interventions while operating under bounded rationality constraints (e.g., limited memory) to rule out brute-force approaches. Under certain assumptions, we show that this reverse engineering goal falls within the class of undecidable problems. Next, we examine some canonical computational systems and reverse engineering goals (as specified by desired I/O behaviors) where reverse engineering can indeed be performed. Finally, using an exemplar network, the ``reward network'' in the brain, we summarize the state of current neuroscientific understanding, and discuss how computer-science and information-theoretic concepts can inform goals of future neuroscience studies.

==> colours.tex <==
\usepackage{xcolor}
%\definecolor{red}{RGB}{204, 0, 0}
%\definecolor{green}{RGB}{51, 153, 51}
%\definecolor{blue}{RGB}{0, 51, 204}
%\definecolor{purple}{RGB}{127, 51, 204}
%\definecolor{orange}{RGB}{255, 102, 0}
\definecolor{red}{HTML}{d62728}
\definecolor{green}{HTML}{2ca02c}
\definecolor{blue}{HTML}{1f77bf}
\definecolor{purple}{HTML}{9467bd}
\definecolor{orange}{HTML}{ff7f0e}
\definecolor{lgray}{HTML}{d7d7d7}


==> nonieee.tex <==
\usepackage{lmodern}

\newcommand{\IEEEoverridecommandlockouts}{}

\newcommand{\IEEEauthorblockN}[1]{#1}
\newcommand{\IEEEauthorblockA}[1]{#1}
\newcommand{\IEEEauthorrefmark}[1]{%
	\ifthenelse{\equal{#1}{1}}%
		{${}^*$}%
		{\ifthenelse{\equal{#1}{2}}%
				{${}^\dagger$}%
				{${}^\ddagger$}%
		}%
}

%\newcommand{\IEEEQED}{$\blacksquare$}
\newcommand{\IEEEQED}{$\square$}
\newcommand{\IEEEQEDopen}{$\square$}

\newenvironment{IEEEproof}{\begin{proof}}{%
    \end{proof}\ignorespacesafterend% as suggested above
}

\newcommand{\appendices}{\appendix}

